Robust Testing in High-Dimensional Sparse Models

We consider the problem of robustly testing the norm of a high-dimensional sparse signal vector under two different observation models. In the first model, we are given $n$ i.i.d. samples from the distribution $\mathcal{N}\left(\theta,I_d\right)$ (with unknown $\theta$), of which a small fraction has been arbitrarily corrupted. Under the promise that $\|\theta\|_0\le s$, we want to correctly distinguish whether $\|\theta\|_2=0$ or $\|\theta\|_2>\gamma$, for some input parameter $\gamma>0$. We show that any algorithm for this task requires $n=\Omega\left(s\log\frac{ed}{s}\right)$ samples, which is tight up to logarithmic factors. We also extend our results to other common notions of sparsity, namely, $\|\theta\|_q\le s$ for any $0 < q < 2$. In the second observation model that we consider, the data is generated according to a sparse linear regression model, where the covariates are i.i.d. Gaussian and the regression coefficient (signal) is known to be $s$-sparse. Here too we assume that an $\epsilon$-fraction of the data is arbitrarily corrupted. We show that any algorithm that reliably tests the norm of the regression coefficient requires at least $n=\Omega\left(\min(s\log d,{1}/{\gamma^4})\right)$ samples. Our results show that the complexity of testing in these two settings significantly increases under robustness constraints. This is in line with the recent observations made in robust mean testing and robust covariance testing.

==> APPENDICES.tex <==
\appendix
\section{Sparse Gaussian mean testing}\label{sec:SGMT}
In this section we provide a proof of the lower bound on the sample complexity of sparse Gaussian mean testing. Define the function $N$ as 
\begin{equation}\label{eqn:smt_sampleCxty}
N(s,d,\gamma)=\begin{cases}
			\frac{s}{\gamma^2}\log\left(1+\frac{d}{s^2}\right) & \text{if  }s<\sqrt{d}\\
            \frac{\sqrt{d}}{\gamma^2} & \text{if  }s\ge \sqrt{d}
		 \end{cases}.    
\end{equation}
\begin{proposition}\label{prop:smt}
Let $\gamma>0$ be fixed. Let $X_1,X_2,\cdots,X_n$ be i.i.d. samples from a distribution $\p$. Then, any algorithm that distinguishes between the cases $\p=\cN(0,I_d)$ and $\p\in\{\cN(\theta,I_d):\normtwo{\theta}\ge\gamma,\norm{\theta}_0\le s\}$ with probability greater than $2/3$ requires $n\ge cN(s,d,\gamma)$, where $N$ is given by (\ref{eqn:smt_sampleCxty}) and $c$ is constant.
\end{proposition}
\begin{proof}
Let $B=\{b\in\{0,1\}^d:\norm{b}_0=s\}$ and $b\sim\text{Uniform}(B)$. Let $\Theta = \frac{\gamma }{\sqrt{s}}B$. With $\q_\theta=\cN(\theta,I_d)$ and $\q=\bE{\theta}{\q_\theta}$, by (\ref{eqn:chi2_div}) we have
\begin{align*}
    1+\chisquare{\q}{G^n} = \bE{\theta,\theta'}{\left(1+\chi^2_{G}(\q_\theta,\q_{\theta'})\right)^n}.
\end{align*}
Since $\q_\theta = \mathcal{N}(\theta,I_d)$, a straightforward computation gives
\begin{equation*}
    1+\chi^2_{G}(\q_\theta,\q_{\theta'}) = \exp(\langle\theta,\theta'\rangle).
\end{equation*}
Thus,
\begin{align*}
    1+\chisquare{\q}{G^n} &= \bE{\theta,\theta'}{\exp(n\langle\theta,\theta'\rangle)}\\
    &= \bE{b,b'}{\exp\left(\frac{n\gamma^2}{s}\langle b,b'\rangle\right)}.
\end{align*}    
By symmetry between $b$ and $b'$ in the above equation, it suffices to evaluate the expectation keeping $b'$ fixed, say at $b_0$. Then the $\langle b,b_0\rangle$ has Hypergeometric distribution. Hence,
\begin{align*}
    1+\chisquare{\q}{G^n} &= \bE{b}{\exp\left(\frac{n\gamma^2}{s}\langle b,b_0\rangle\right)}\\
    &= \expect{\exp\left(\frac{n\gamma^2}{s}H\right)},
\end{align*}
where $H\sim\hypergeom(d,s,s)$. Let $B\sim$Binomial$(s,\frac{s}{d})$. Then by Theorem~23.1 in \cite{Wu20}, we have
\begin{equation*}
    \expect{\exp(\lambda H)}\le \expect{\exp(\lambda B)} = \left(1+\frac{s}{d}(e^\lambda-1)\right)^s.
\end{equation*}
Thus,
\begin{align*}
    \chisquare{\q}{G^n} &\le \left(1+\frac{s}{d}(e^{\frac{n\gamma^2}{s}}-1)\right)^s-1\\
    &\le \exp\left(\frac{s^2}{d}(e^{\frac{n\gamma^2}{s}}-1)\right)-1.
\end{align*}
Therefore, for $\chisquare{\q}{G^n}$ to be $\Omega(1)$, we need $n=\Omega\left(\frac{s}{\gamma^2}\log\left(1+\frac{d}{s^2}\right)\right)$. For $s=\sqrt{d}$, we get $n=\Omega\left(\frac{\sqrt{d}}{\gamma^2}\right)$. By construction, the sample complexity at lower values of $s$ is a lower bound for higher values of $s$. Hence, we have $n=\Omega\left(\frac{\sqrt{d}}{\gamma^2}\right)$ for $s\ge\sqrt{d}$.   
\end{proof}
\begin{remark}
The sample complexity in Proposition~\ref{prop:smt} turns out to be tight. Let $\hat{\theta}\eqdef \frac{1}{n}\sum_{i=1}^n X_i$ and $\alpha \eqdef \expectCond{Y^2}{Y^2>\beta^2}$, where $Y\sim \cN(0,1)$ and $\beta = \sqrt{2\log(1+d/s^2)}$. Define the statistic $\hat{T}$ as $\hat{T} = \sqrt{\max\{\hat{S},0\}}$, where 
\begin{equation*}
    \hat{S} = \begin{cases}
			\sum_{j=1}^d (\hat{\theta}_j^2-\alpha/n)\mathds{1}_{\left\{|\hat{\theta}_j|>
			\frac{\beta}{\sqrt{n}}\right\}} & \text{if  }s<\sqrt{d}\\
            	\sum_{j=1}^d \hat{\theta}_j^2-d/n & \text{if  }s\ge \sqrt{d}
		 \end{cases}.  
\end{equation*}
The test $\hat{T}\ge\gamma/2$ achieves the lower bound given in Proposition~\ref{prop:smt} \cite{Olivier17}.
\end{remark}

